LUTNet: Rethinking Inference in FPGA Soft Logic

Research has shown that deep neural networks contain significant redundancy, and that high classification accuracies can be achieved even when weights and activations are quantised down to binary values. Network binarisation on FPGAs greatly increases area efficiency by replacing resource-hungry multipliers with lightweight XNOR gates. However, an FPGA's fundamental building block, the K-LUT, is capable of implementing far more than an XNOR: it can perform any K-input Boolean operation. Inspired by this observation, we propose LUTNet, an end-to-end hardware-software framework for the construction of area-efficient FPGA-based neural network accelerators using the native LUTs as inference operators. We demonstrate that the exploitation of LUT flexibility allows for far heavier pruning than possible in prior works, resulting in significant area savings while achieving comparable accuracy. Against the state-of-the-art binarised neural network implementation, we achieve twice the area efficiency for several standard network models when inferencing popular datasets. We also demonstrate that even greater energy efficiency improvements are obtainable.

==> diagrams/BNN.tex <==
\begin{tikzpicture}[label distance=2mm,decoration={markings,mark= at position 0.5 with{\node[font=\footnotesize] {/};} },scale=0.4, every node/.style={scale=0.6}]


    \tikzstyle{ActBox} = [rectangle, fill=white, fill opacity=1, draw, text centered, minimum height=2em, minimum width=2em, node distance=3cm, text width=2.2em]
    \tikzstyle{WeiBox} = [rectangle, draw, text centered, minimum height=2em, minimum width=2em, node distance=3cm, text width=2em]
    \tikzstyle{FuncBox} = [rectangle, draw, text centered, minimum height=1em, minimum width=2em, node distance=3cm, text width=3em]
    \tikzstyle{OpCirc} = [circle, draw, text centered, minimum width=2em, node distance=3cm, text width=1.4em]
    \tikzstyle{TextBox} = [rectangle, text centered, minimum height=1em, minimum width=10em, node distance=3cm, text width=9em]
    
    \node[WeiBox] at (0.8,6.5) (w111) {$w_{1}$};
    \node[WeiBox] at (0.8,5.0) (w211) {$w_{2}$};
    \node[WeiBox] at (0.8,3.5) (w311) {$w_{3}$};
    \node[WeiBox] at (0.8,1.) (w411) {$w_{N}$};
    
    \node[ActBox] at ($(w111)+(-1.2,-0.8)$) (x11) {$x_1$};
    \node[ActBox] at ($(w211)+(-1.2,-0.8)$) (x21) {$x_2$};
    \node[ActBox] at ($(w311)+(-1.2,-0.8)$) (x31) {$x_3$};
    \node[ActBox] at ($(w411)+(-1.2,-0.8)$) (x41) {$x_N$};
    
    \node[xnor gate US, draw, minimum height=1.5em] at ($(w111)+(1.8,-0.3)$) (mul1) {};
    \node[xnor gate US, draw, minimum height=1.5em] at ($(w211)+(1.8,-0.3)$) (mul2) {};
    \node[xnor gate US, draw, minimum height=1.5em] at ($(w311)+(1.8,-0.3)$) (mul3) {};
    \node[xnor gate US, draw, minimum height=1.5em] at ($(w411)+(1.8,-0.3)$) (mul4) {};
    
    \node[TextBox] at ($(w311)+(0.2,-1.2)$) (dots1) {$\vdots$};
    
    \draw [->] (w111.east) -| ($(w111.east)+(0.2,0)$) |- (mul1.input 1);
    \draw [->] (x11.east) -| ($(x11.east)+(1.3,0)$) |- (mul1.input 2);
    \draw [->] (w211.east) -| ($(w211.east)+(0.2,0)$) |- (mul2.input 1);
    \draw [->] (x21.east) -| ($(x21.east)+(1.3,0)$) |- (mul2.input 2);
    \draw [->] (w311.east) -| ($(w311.east)+(0.2,0)$) |- (mul3.input 1);
    \draw [->] (x31.east) -| ($(x31.east)+(1.3,0)$) |- (mul3.input 2);
    \draw [->] (w411.east) -| ($(w411.east)+(0.2,0)$) |- (mul4.input 1);
    \draw [->] (x41.east) -| ($(x41.east)+(1.3,0)$) |- (mul4.input 2);
    
    \node[rectangle, draw, minimum height=2em] at ($(mul2)+(2,-0.5)$) (sum1) {$\sum$};
    
    \draw [->] (mul1.output) -| ($(mul1.output)+(0.4,0)$) |- ($(sum1.west)+(0,0.3)$);
    \draw [->] (mul2.output) -| ($(mul2.output)+(0.2,0)$) |- ($(sum1.west)+(0,0.1)$);
    \draw [->] (mul3.output) -| ($(mul3.output)+(0.2,0)$) |- ($(sum1.west)+(0,-0.1)$);
    \draw [->] (mul4.output) -| ($(mul4.output)+(0.4,0)$) |- ($(sum1.west)+(0,-0.3)$);
    
    \draw [->,postaction={decorate}] (sum1.east) -- ($(sum1)+(1,0)$);
    % \node[ActBox] at ($(thresh1)+(1.5,0)$) (x12) {$x_1^{(l+1)}$};
    % \draw [->,postaction={decorate}] (thresh1.east) -- (x12.west);
    
    \node[TextBox] at ($(sum1)+(0,-1)$) (dots2) {$\vdots$};
    
    % Draw a huge hollowed arrow
    
    \node at ($(sum1)+(2,1)$) (arrow){};
    \draw (arrow.east) -- ($(arrow.east)+(0,-2)$) -- ($(arrow.east)+(0.25,-2)$) -- ($(arrow.east)+(0.25,-2.5)$) -- ($(arrow.east)+(1,-1)$) -- ($(arrow.east)+(0.25,0.5)$) -- ($(arrow.east)+(0.25,0)$) -- (arrow.east);
    
    % Invisible node for shifting position
    
    \node at (-2,3) (invisible){};

\end{tikzpicture}

==> diagrams/LUTNet.tex <==
\begin{tikzpicture}[label distance=2mm,decoration={markings,mark= at position 0.5 with{\node[font=\footnotesize] {/};} },scale=0.4, every node/.style={scale=0.6}]


    \tikzstyle{ActBox} = [rectangle, fill=white, fill opacity=1, draw, text centered, minimum height=1em, minimum width=2em, node distance=3cm, text width=2em]
    \tikzstyle{WeiBox} = [rectangle, draw, text centered, minimum height=1em, minimum width=3.8em, node distance=3cm, text width=4.8em]
    \tikzstyle{FuncBox} = [rectangle, draw, text centered, minimum height=1em, minimum width=2em, node distance=3cm, text width=3em]
    \tikzstyle{OpCirc} = [circle, draw, text centered, minimum width=2em, node distance=3cm, text width=1.4em]
    \tikzstyle{TextBox} = [rectangle, text centered, minimum height=1em, minimum width=10em, node distance=3cm, text width=9em]
    
    \node[WeiBox] at (2.3,6.5) (w111) {$\tilde{x}_1^{\left(1\right)}=x_1$};
    % \node[WeiBox] at (0.8,5.5) (w211) {$\tilde{x}_2^{\left(2\right)}$};
    \node[WeiBox] at (2.3,3.5) (w311) {$\tilde{x}_1^{\left(2\right)}=x_3$};
    \node[WeiBox] at (2.3,1) (w411) {$\tilde{x}_1^{\left(\tilde{N}\right)}=x_{\tilde{N}}$};
    
    \node[ActBox] at ($(w111)+(-2,-0.8)$) (x11) {$\tilde{x}_2^{\left(1\right)}$};
    % \node[ActBox] at ($(w211)+(-1.3,-0.5)$) (x21) {$\tilde{x}_2^{\left(2\right)}=x_2$};
    \node[ActBox] at ($(w311)+(-2,-0.8)$) (x31) {$\tilde{x}_2^{\left(2\right)}$};
    \node[ActBox] at ($(w411)+(-2,-0.8)$) (x41) {$\tilde{x}_2^{\left(\tilde{N}\right)}$};
    
    \node[rectangle, draw, minimum height=2em, minimum width=4em] at ($(w111)+(3.2,-0.3)$) (mul1) {2-LUT};
    \node[xnor gate US, draw, minimum height=1.5em] at ($(w111)+(3.2,-1.8)$) (mul2) {};
    \node[rectangle, draw, minimum height=2em, minimum width=4em] at ($(w311)+(3.2,-0.3)$) (mul3) {2-LUT};
    \node[rectangle, draw, minimum height=2em, minimum width=4em] at ($(w411)+(3.2,-0.3)$) (mul4) {2-LUT};
    
    \draw[red] ($(mul2)+(0.5,0.5)$) -- ($(mul2)+(-0.5,-0.5)$);
    \draw[red] ($(mul2)+(-0.5,0.5)$) -- ($(mul2)+(0.5,-0.5)$);
    
    \node[TextBox] at ($(w311)+(0.2,-1.2)$) (dots1) {$\vdots$};
    
    \draw [->] (w111.east) -| ($(w111.east)+(0.2,0)$) |- ($(mul1.north west)+(0,-0.25)$);
    \draw [->] (x11.east) -| ($(x11.east)+(3,0)$) |- ($(mul1.south west)+(0,0.25)$);
    % \draw [->] (w211.east) -| ($(w211.east)+(0.2,0)$) |- (mul2.input 1);
    % \draw [->] (x21.east) -| ($(x21.east)+(1.2,0)$) |- (mul2.input 2);
    \draw [->] (w311.east) -| ($(w311.east)+(0.2,0)$) |- ($(mul3.north west)+(0,-0.25)$);
    \draw [->] (x31.east) -| ($(x31.east)+(3,0)$) |- ($(mul3.south west)+(0,0.25)$);
    \draw [->] (w411.east) -| ($(w411.east)+(0.2,0)$) |- ($(mul4.north west)+(0,-0.25)$);
    \draw [->] (x41.east) -| ($(x41.east)+(3,0)$) |- ($(mul4.south west)+(0,0.25)$);
    
    \node[rectangle, draw, minimum height=2em] at ($(mul2)+(2.4,-0.5)$) (sum1) {$\sum$};
    
    \draw [->] (mul1.east) -| ($(mul1.east)+(0.4,0)$) |- ($(sum1.west)+(0,0.3)$);
    % \draw [->] (mul2.output) -| ($(mul2.output)+(0.2,0)$) |- ($(sum1.west)+(0,0.1)$);
    \draw [->] (mul3.east) -| ($(mul3.east)+(0.2,0)$) |- ($(sum1.west)+(0,-0.1)$);
    \draw [->] (mul4.east) -| ($(mul4.east)+(0.4,0)$) |- ($(sum1.west)+(0,-0.3)$);
    
    \draw [->,postaction={decorate}] (sum1.east) -- ($(sum1)+(1,0)$);
    
    \node[TextBox] at ($(sum1)+(0,-1)$) (dots2) {$\vdots$};
    
    % Invisible node for shifting position
    
    \node at (-3,2) (invisible){};
    

\end{tikzpicture}

==> diagrams/transform_doublecol.tex <==
\begin{tikzpicture}[node distance=0.25cm, thick, circuit logic US]
	
	\newcommand{\updownkinklen}{0.2cm}
	\newcommand{\leftkinklen}{0.25cm}
	\newcommand{\upperinputlen}{1cm}
	\newcommand{\lowerinputlen}{0.25cm}
	\newcommand{\rightkinklen}{0.25cm}
	\newcommand{\outputlen}{0.5cm}
	
	\tikzstyle {xnor} = [xnor gate, point right, inputs={nn}]
	\tikzstyle {lut} = [rectangle, minimum width=1.5cm, minimum height=0.75cm, align=center, draw]
	\tikzstyle {sum} = [circle, minimum width=0.75cm, minimum height=0.75cm, align=center, draw]
	\tikzstyle {act} = [rectangle, minimum width=0.75cm, minimum height=0.75cm, align=center, draw]
	\tikzstyle {arrow} = [->, >=stealth]
	
	\node (lut3) [lut] {2-LUT};
	\node (lut2) [lut, above=of lut3, white] {2-LUT};
	\node (pruned) [xnor] at (lut2) {};
	\node (lut1) [lut, above=of lut2] {2-LUT};
	\node (lut4) [lut, below=of lut3, white] {};
	\node at ([yshift=0.1cm]lut4) {$\vdots$};
	\node (lut5) [lut, below=of lut4] {2-LUT};
	\node (sum2) [sum, right=of lut3, xshift=0.25cm] {$\Sigma$};
	\node (act2) [act, right=of sum2, xshift=0.75cm] {$f$};
	
	\node (to) [left=of lut3, xshift=-4cm] {};
	\draw [fill=black] ([xshift=-0.5cm, yshift=-0.5cm]to.center) -- ([xshift=-0.5cm, yshift=0.5cm]to.center) -- ([yshift=0.5cm]to.center) -- ([yshift=0.75cm]to.center) -- ([xshift=0.5cm]to.center) -- ([yshift=-0.75cm]to.center) -- ([yshift=-0.5cm]to.center) -- cycle;
	
	\node (act1) [act, left=of to, xshift=-2cm] {$f$};
	\node (sum1) [sum, left=of act1, xshift=-0.75cm] {$\Sigma$};
	\node (xnor3) [xnor, left=of sum1, xshift=-0.25cm] {};
	\node (xnor1) [xnor] at (lut1 -| xnor3) {};
	\node (xnor2) [xnor] at (lut2 -| xnor3) {};
	\node at ([yshift=0.1cm]lut4 -| xnor3) {$\vdots$};
	\node (xnor5) [xnor] at (lut5 -| xnor3) {};
	
	\draw [red] ([xshift=-0.5cm, yshift=-0.5cm]pruned.center) -- ([xshift=0.5cm, yshift=0.5cm]pruned.center);
	\draw [red] ([xshift=-0.5cm, yshift=0.5cm]pruned.center) -- ([xshift=0.5cm, yshift=-0.5cm]pruned.center);
	
	\draw (xnor1.input 1 -| lut1.west) -- ++(left:\leftkinklen) -- ++(up:\updownkinklen) -- ++(left:\upperinputlen) node [left, anchor=east] {$\tilde{x}_1^{\left(1\right)} = x_1$};
	\draw (xnor1.input 2 -| lut1.west) -- ++(left:\leftkinklen) -- ++(down:\updownkinklen) -- ++(left:\lowerinputlen) node [left, anchor=east] {$\tilde{x}_2^{\left(1\right)}$};
	\draw (xnor3.input 1 -| lut3.west) -- ++(left:\leftkinklen) -- ++(up:\updownkinklen) -- ++(left:\upperinputlen) node [left, anchor=east] {$\tilde{x}_1^{\left(2\right)} = x_3$};
	\draw (xnor3.input 2 -| lut3.west) -- ++(left:\leftkinklen) -- ++(down:\updownkinklen) -- ++(left:\lowerinputlen) node [left, anchor=east] {$\tilde{x}_2^{\left(2\right)}$};
	\draw (xnor5.input 1 -| lut5.west) -- ++(left:\leftkinklen) -- ++(up:\updownkinklen) -- ++(left:\upperinputlen) node [left, anchor=east] {$\tilde{x}_1^{\left(\tilde{N}\right)} = x_N$};
	\draw (xnor5.input 2 -| lut5.west) -- ++(left:\leftkinklen) -- ++(down:\updownkinklen) -- ++(left:\lowerinputlen) node [left, anchor=east] {$\tilde{x}_2^{\left(\tilde{N}\right)}$};
	\draw [arrow] (lut1.east) -- ++(right:\rightkinklen) -- (sum2);
	\draw [arrow] (lut3.east) -- ++(right:\rightkinklen) -- (sum2);
	\draw [arrow] (lut5.east) -- ++(right:\rightkinklen) -- (sum2);
	\draw (sum2) -- (act2.west);
	\draw ([xshift=-0.1cm, yshift=-0.1cm]$(sum2.east)!0.5!(act2.west)$) -- ([xshift=0.1cm, yshift=0.1cm]$(sum2.east)!0.5!(act2.west)$) node [midway, above, anchor=west, rotate=90, xshift=0.1cm] {$\left\lceil\log_2{\left(\tilde{N}\right)}\right\rceil$};
	\draw (act2.east) -- ++(right:\outputlen) node [right, anchor=west] {$y$};
	
	\draw (xnor1.input 1) -- ++(left:\leftkinklen) -- ++(up:\updownkinklen) -- ++(left:\upperinputlen) node [left, anchor=east] {$x_1$};
	\draw (xnor1.input 2) -- ++(left:\leftkinklen) -- ++(down:\updownkinklen) -- ++(left:\lowerinputlen) node [left, anchor=east] {$w_1$};
	\draw (xnor2.input 1) -- ++(left:\leftkinklen) -- ++(up:\updownkinklen) -- ++(left:\upperinputlen) node [left, anchor=east] {$x_2$};
	\draw (xnor2.input 2) -- ++(left:\leftkinklen) -- ++(down:\updownkinklen) -- ++(left:\lowerinputlen) node [left, anchor=east] {$w_2$};
	\draw (xnor3.input 1) -- ++(left:\leftkinklen) -- ++(up:\updownkinklen) -- ++(left:\upperinputlen) node [left, anchor=east] {$x_3$};
	\draw (xnor3.input 2) -- ++(left:\leftkinklen) -- ++(down:\updownkinklen) -- ++(left:\lowerinputlen) node [left, anchor=east] {$w_3$};
	\draw (xnor5.input 1) -- ++(left:\leftkinklen) -- ++(up:\updownkinklen) -- ++(left:\upperinputlen) node [left, anchor=east] {$x_N$};
	\draw (xnor5.input 2) -- ++(left:\leftkinklen) -- ++(down:\updownkinklen) -- ++(left:\lowerinputlen) node [left, anchor=east] {$w_N$};
	\draw [arrow] (xnor1.output) -- ++(right:\rightkinklen) -- (sum1);
	\draw [arrow] (xnor2.output) -- ++(right:\rightkinklen) -- (sum1);
	\draw [arrow] (xnor3.output) -- ++(right:\rightkinklen) -- (sum1);
	\draw [arrow] (xnor5.output) -- ++(right:\rightkinklen) -- (sum1);
	\draw (sum1) -- (act1.west);
	\draw ([xshift=-0.1cm, yshift=-0.1cm]$(sum1.east)!0.5!(act1.west)$) -- ([xshift=0.1cm, yshift=0.1cm]$(sum1.east)!0.5!(act1.west)$) node [midway, above, anchor=west, rotate=90, xshift=0.1cm] {$\left\lceil\log_2{\left(N\right)}\right\rceil$};
	\draw (act1.east) -- ++(right:\outputlen) node [right, anchor=west] {$y$};
	
\end{tikzpicture}

